Sensitivity to Unobserved Confounding in Studies with Factor-structured Outcomes

In this work, we propose an approach for assessing sensitivity to unobserved confounding in studies with multiple outcomes. We demonstrate how prior knowledge unique to the multi-outcome setting can be leveraged to strengthen causal conclusions beyond what can be achieved from analyzing individual outcomes in isolation. We argue that it is often reasonable to make a shared confounding assumption, under which residual dependence amongst outcomes can be used to simplify and sharpen sensitivity analyses. We focus on a class of factor models for which we can bound the causal effects for all outcomes conditional on a single sensitivity parameter that represents the fraction of treatment variance explained by unobserved confounders. We characterize how causal ignorance regions shrink under additional prior assumptions about the presence of null control outcomes, and provide new approaches for quantifying the robustness of causal effect estimates. Finally, we illustrate our sensitivity analysis workflow in practice, in an analysis of both simulated data and a case study with data from the National Health and Nutrition Examination Survey (NHANES).

==> sections/aging_clock.tex <==
\section{Analysis of Metabolomic Aging Clocks}
\label{sec:age-metabolite-analysis}


In this section, we demonstrate our method in analysis of the effect of age on small molecules, called ``metabolites", in humans. The metabolome consists of the structural and functional building blocks of an organism, which bridges genotype and phenotype and plays an important role in studies of aging and age-related traits \citep{hwangbo2021aging}. We utilize targeted metabolomics dataset from \citet{hwangbo2021aging} to investigate how aging affects the concentration of metabolites in cerebrospinal fluid (CSF). We focus on the analysis of 39 targeted metabolites measured for 85 individuals, and their corresponding age, ranging from 20 to 86 years old at time of healthy sample collection. We follow the data pre-processing used by \citep{hwangbo2021aging} and use the R package $\texttt{Amelia}$ to impute the missing values. We let $T$ denote the age and $Y = (Y_1, \cdots, Y_{39})$ be the measured concentration of targeted metabolites in CSF. Our estimand of interest is the biological effect of one year increase in age on each metabolite. 

Inferring the biological effect of aging on the metabolome can be complicated by experimental confounders other sources of unwanted biological variation \citep{livera2015statistical}. For example, in their original analysis \citet{hwangbo2021aging} did not take into account the time between sample collection and the mass spectrometry-based assay to measure abundances of metabolites.  Although not some studies indicate that long term storage may lead to significant decay among many metabolites \citep{haid2018long}.  Unfortunately, samples from all subjects under 40 years of age were collected in the first 3 years of the study, whereas samples from older individuals were collected nearly uniformly over an 8 year time period.  





% For instance, younger people tend to exercise more than seniors, and exercise is known to significantly affect concentrations of some metabolites, such as lactate, pyruvate, TCA cycle intermediates \citep{schranner2020metabolite}. 

For simplicity, we model the outcome model with a linear regression, although other flexible outcome models like $\texttt{BART}$ are also applicable \citep{chipman2010bart}. With the linear assumption, our estimand reduces to the regression coefficient, $\tau_j$, which is invariant to the specific level of $t_1$ and $t_2$, i.e., our estimand is
\begin{equation}
\label{eqn:estimand-age-metabolite}
    \text{PATE}_{e_j} = \tau_j
\end{equation}
for all $j = 1, \cdots, q$, and all $t_1, t_2$ such that $t_1 - t_2 = 1$. We rescale all outcomes to unit variance and regress the scaled outcomes on age to estimate $\tau^{\text{naive}}_j$ under an assumption of no unobserved confounding, and we apply factor analysis using the R function $\texttt{factanal}$ to the residual outcomes. We use cross validation to select the latent confounder dimension $m = 3$. First, we compute the ignorance regions of the treatment effects for all metabolites assuming $R^2_{T \sim U} \leq 95\%$ without incorporating any null or non-null control assumptions. As a result, all ignorance regions contain zero, which suggests that their treatment effects are sensitive to the unobserved confounding (see Figure \ref{fig:meta_ig_all}). 
In Table \ref{table:rv_meta} of the Appendix, we include robustness values for each metabolite, where the median is at 22\% and the maximum is at 87\% for glycerol 3-phosphate.
In the following, we show that, by making use of the null or non-null control outcomes, we can further shrink the ignorance regions and make some of the metabolites with significant treatment effects distinguishable from the others.
% To validate our analysis, we compare the calibrated effect estimates to the conclusions drawn in \citep{hwangbo2021aging}. 



\vspace*{12pt}
\noindent \textbf{Calibration with null controls.} Following the discussion in Section \ref{sec:cali_wnco}, we demonstrate the validity of our calibration method with null control outcomes.
To demonstrate our approach, we use sorbitol, a sugar substitute, as a null control, as it has a reduced tendency to increase the sugar level in the blood and is used by diabetes patients and elderly individuals \citep{gabbay1973sorbitol} \footnote{We do not claim that sorbitol }. 

We plot the ignorance regions before and after the calibration with the null control, ordered by the extent to which they are influence by the non-null calibration (Figure \ref{fig:cali_wnco}). 
The ignorance region is constructed using 95\% confidence interval for $\tau^{\text{naive}}$
in order to account for the estimation uncertainty of the observed data distribution.
With the additional information about confounders provided by the null control, the ignorance region is largely reduced for treatment effects of the first few metabolites on the left in plot \ref{fig:cali_wnco}. Also, the estimate under the nonconfoundedness assumption (i.e. $R^2_{T \sim U} = 0$) for each metabolite changes after taking the null control outcome into account. Notably, we find that, after adjusting sorbitol to have a zero treatment effect, the effect of age on 
alpha-ketoisovaleric acid
% 4-Methylvaleric acid, alpha-ketoisovaleric acid, Glycohyodeoxycholic acid, Glycoursodeoxycholic acid, Fructose, Levulinic acid, Glycocyamine, alpha-Hydroxyisovaleric acid, Glycochenodeoxycholate, Mannose, Glycodeoxycholic acid, Citraconic acid and Lactate 
becomes robustly negative at level $R^2_{T \sim U} = 95\%$.
% , while the age effect on Anthranilic acid becomes robustly positive at level $R^2_{T \sim U} = 95\%$.
% , which are respectively claimed to have null and positive treatment effects in \citep{hwangbo2021aging}.

\begin{figure}
    \centering
    \includegraphics[width = \textwidth]{figs/metabolite_robustness.pdf}
    \caption{Robustness values for metabolites, before and after considering sortibol as a null control outcome.  Reported values are the lower end point of the 95\% posterior credible region for the robustness value.  Note that while sorbitol is significant under NUC, the lower endpoing of the robustness value is only $RV = 0.02$, which suggests that it is sensitive to confounding.  Despite this small value, after enforcing the null control assumption, the robustness values for all other metabolites increase, often by much more than 0.02.}
    \label{fig:cali_wnco}
\end{figure}

Latent mediators include factors related to diet, exercise and lifestyle.  The metabolome is known to be particularly sensitive to diet


==> sections/multi_t_and_multi_o.tex <==
We have demonstrated that in model \ref{eqn:confounder}-\ref{eqn:outcome} with multivariate treatments, the confounder-treatment relationship, parameterized by $B$, is identifiable up to a causal equivalence class, while the confounder-outcome relationship, parameterized by $\gamma$ is unidentifiable. On the contrary, in model \ref{eqn:confounder,multi-y}-\ref{eqn:outcome,multi-y} with multivariate outcomes, the confounder-outcome relationship, parameterized by $\Gamma$, is identifiable up to a causal equivalence class, while the confounder-treatment relationship, characterized by $\beta$, is unidentifiable. In parallel, we explore the answer with the following linear model:
\begin{align}
    U &= \epsilon_u,  \quad \epsilon_u \sim N_m(0, \ I_m \otimes I_n), \label{eqn:confounder,multi-ty}\\
    T &= BU + \epsilon_{t|u}, \quad \epsilon_{t|u} \sim N_k(0, \ \sigma_{t|u}^2 I_k \otimes I_n), \label{eqn:treatment,multi-ty}\\
    Y &= \Tau T + \Gamma U + \epsilon_{y|t,u}, \quad \epsilon_{y|t,u} \sim N_q(0, \ \sigma_{y|t,u}^2 I_q \otimes I_n), \label{eqn:outcome,multi-ty},
\end{align}
where $B$, $\Tau$ and $\Gamma$ are respectively $k \times m$, $q \times k$ and $q \times m$ matrices. Note that, in the above model, the treatment assignment mechanism defined in Equation \ref{eqn:treatment,multi-ty} is same as the one in model \ref{eqn:confounder}-\ref{eqn:outcome}, where the conditional confounder distribution $f(u \mid t) \sim N(\mu_{u|t}, \ \Sigma_{u|t})$ is identifiable, with $\mu_{u|t}$ and $\Sigma_{u|t}$ as known functions of $B$ and $\sigma_{t|u}^2$. Additionally, as the outcomes are multivariate in Equation \ref{eqn:outcome,multi-ty}, the confounder-outcome relationship, characterized by $\Gamma$, can also be identified according to the discussion of Section \ref{sec:copula-based_sens_analy_gaussian_copula,multi-y}. 

Under model \ref{eqn:confounder,multi-ty}-\ref{eqn:outcome,multi-ty}, the intervention distribution has density
\begin{equation}
    f(y \mid do(T = t)) \sim N(\Tau T,  \ \sigma_{y|t, u}^2 I_q + \Gamma \Sigma_u \Gamma'),
\end{equation}
and the observed outcome distribution can be written as 
\begin{equation}
    f(T \mid T = t) \sim N_q(\Tau^{\text{naive}}t, \ \Sigma_{y|t}),
\end{equation}
where 
\begin{align}
    % \mu_{u|t} &= \Sigma_u B'( B\Sigma_u B' + \sigma_{t|u}^2 I_{k})^{-1}t,\\
    % \Sigma_{u|t} &= \Sigma_u - \Sigma_u B'(B \Sigma_u B' + \sigma_{t|u}^2 I_k)^{-1} B \Sigma_u,\\
    \Tau^{\text{naive}}t &= \Tau t + \Gamma \Sigma_u B'( B\Sigma_u B' + \sigma_{t|u}^2 I_{k})^{-1}t\\
    &= \Tau t + \Gamma \mu_{u|t},\\
    \Sigma_{y|t} &= \sigma_{y|t, u}^2 I_q + \Gamma(\Sigma_u - \Sigma_u B'(B \Sigma_u B' + \sigma_{t|u}^2 I_k)^{-1} B \Sigma_u) \Gamma',\\
    &= \sigma_{y|t, u}^2 I_q + \Gamma \Sigma_{u|t} \Gamma',
\end{align}
which are fully identifiable. 

For given $t_1, t_2$, our estimand of interest, $\text{PATE}_{t_1,t_2}$, can be written as a function of only the identifiable terms:
\begin{align}
    \text{PATE}_{t_1,t_2} &= \Tau(t_1 - t_2),\\
    &= \Tau^{\text{naive}}t - \Gamma \mu_{u|t},
\end{align}
which indicates that the treatment effects is identifiable when both treatments and outcomes are multivariate.



